Data Efficient Human Intention Prediction: Leveraging Neural Network Verification and Expert Guidance

Predicting human intention is critical to facilitating safe and efficient human-robot collaboration (HRC). However, it is challenging to build data-driven models for human intention prediction. One major challenge is due to the diversity and noise in human motion data. It is expensive to collect a massive motion dataset that comprehensively covers all possible scenarios, which leads to the scarcity of human motion data in certain scenarios, and therefore, causes difficulties in constructing robust and reliable intention predictors. To address the challenge, this paper proposes an iterative adversarial data augmentation (IADA) framework to learn neural network models from an insufficient amount of training data. The method uses neural network verification to identify the most "confusing" input samples and leverages expert guidance to safely and iteratively augment the training data with these samples. The proposed framework is applied to collected human datasets. The experiments demonstrate that our method can achieve more robust and accurate prediction performance compared to existing training methods.

==> plots/training_time.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.1,0,0.95}
\definecolor{color1}{rgb}{1,0,0}
\definecolor{color2}{rgb}{1,0.498,0.0549}
\pgfplotsset{compat=1.5}
\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
width = 0.36\linewidth,
height = 3.5cm,
font = \small,%\footnotesize,
legend cell align={left},
legend style={nodes={scale=0.5, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=inside,
tick pos=left,
xmin=0, xmax=5100,
xtick style={color=black},
% xlabel={Training Epochs},
ylabel={Time (s)},
ymin=0, ymax=750,
ytick style={color=black}
%title = {Training Time}
]
\addplot [thick, color0]
table {%
0 0
500 6.453
1000 13.946
2000 32.423
3000 54.682
4000 80.866
5000 110.937
};
\addlegendentry{REG}

\addplot [thick, color2]
table {%
0 0
500 12.320
1000 24.909
2000 45.960
3000 64.942
4000 83.926
5000 112.354
};
\addlegendentry{COAP}

\addplot [thick, color1]
table {%
0 0
500 6.294
1000 34.700
2000 160.04
3000 303.297
4000 516.305
5000 738.713

};
\addlegendentry{IADA}




\nextgroupplot[
width = 0.36\linewidth,
height = 3.5cm,
font = \small,
legend cell align={left},
legend style={nodes={scale=0.5, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=inside,
tick pos=left,
xmin=0, xmax=5100,
xtick style={color=black},
xlabel={Training Epochs},
% ylabel={Time (s)},
ymode=log,
log basis y={10},
ymin=0, ymax=40000,
ytick style={color=black}
%title = {Training Time}
]

\addplot [thick, color0]
table {%
0 0
500 25.056
1000 50.179
2000 100.500
3000 151.087
4000 201.304
5000 251.703
};
\addlegendentry{REG}

\addplot [thick, color2]
table {%
0 0
500 30.962
1000 62.157
2000 125.018
3000 187.88
4000 250.856
5000 313.673
};
\addlegendentry{COAP}

\addplot [thick, color1]
table {%
0 0
500 2038.587
1000 4996.280
2000 11402.792
3000 16854.147
4000 21942.204
5000 27156.573

};
\addlegendentry{IADA}




\nextgroupplot[
width = 0.36\linewidth,
height = 3.5cm,
font = \small,
legend cell align={left},
legend style={nodes={scale=0.5, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=inside,
tick pos=left,
xmin=0, xmax=1600,
xtick style={color=black},
% xlabel={Training Epochs},
%ylabel={Time (s)},
ymode=log,
log basis y={10},
ymin=0, ymax=40000,
ytick style={color=black}
%title = {Training Time}
]

\addplot [thick, color0]
table {%
0 0
50 5.51
100 9.66
500 41.34
1000 71.49
1500 105.31
};
\addlegendentry{REG}

\addplot [thick, color2]
table {%
0 0
50 38
100 61
500 288
1000 496
1500 680
};
\addlegendentry{COAP}

\addplot [thick, color1]
table {%
0 0
50 396
100 678
500 2967
1000 4932
1500 6800
};
\addlegendentry{IADA}






\end{groupplot}
\end{tikzpicture}


==> plots/true_adv_percentage.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.1,0,0.95}
\definecolor{color1}{rgb}{1,0,0}
\definecolor{color2}{rgb}{1,0.498,0.0549}
\pgfplotsset{compat=1.5}
\begin{groupplot}[group style={group size=1 by 2}]
\nextgroupplot[
width = \linewidth,
height = 3cm,
font = \small,
legend cell align={left},
legend style={nodes={scale=0.5, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=inside,
tick pos=left,
xmin=0, xmax=4100,
xtick style={color=black},
xlabel={Training Epochs},
ylabel={Percentage},
ymin=0.0, ymax=1.1,
ytick style={color=black},
%title = {Percentage of True Adversarial Data}
]
\addplot [thick, color0]
table {%
0 0
500 0.7072
1000 0.5060
1500 0.4752
2000 0.5078
2500 0.5249
3000 0.5563
3500 0.5302
4000 0.5479
};
\addlegendentry{2D Binary Classification}

\addplot [thick, color2]
table {%
0 0
500 1
1000 1
1500 1
2000 1
2500 1
3000 1
3500 1
4000 1
};
\addlegendentry{MNIST}
\addplot [thick, color1]
table {%
0 0
500 0.1037
1000 0.4250
1500 0.5363
2000 0.4210
2500 0.5814
3000 0.4914
3500 0.3922
4000 0.5966

};
\addlegendentry{Intention Prediction}

\end{groupplot}


\end{tikzpicture}


==> supplement_img/C_Qv_D.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.1,0,0.95}
\definecolor{color1}{rgb}{1,0,0}
\definecolor{color2}{rgb}{1,0.498,0.0549}
\pgfplotsset{compat=1.5}
\begin{groupplot}[group style={group size=2 by 1, horizontal sep=60pt}]
\nextgroupplot[
width = 0.48\linewidth,
height = 4.5cm,
font = \small,%\footnotesize,
legend cell align={left},
legend style={nodes={scale=0.5, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=inside,
tick pos=left,
xmin=1000, xmax=5000,
xtick style={color=black},
xlabel={Number of Seeds ($C$)},
ylabel={Level of Expansion},
% ymode=log,
% log basis y={10},
ymin=0, ymax=9,
ytick style={color=black}
%title = {Training Time}
]
\addplot [thick, color0]
table {%
1000 4
2000 5
5000 5
};
\addlegendentry{2D Classification}

\addplot [thick, color1]
table {%
1000 4
2000 5
5000 6
};
\addlegendentry{Robot Handover}

\addplot [thick, color2]
table {%
1000 1
2000 2
5000 3
};
\addlegendentry{Human Assembly}


\nextgroupplot[
width = 0.48\linewidth,
height = 4.5cm,
font = \small,%\footnotesize,
legend cell align={left},
legend style={nodes={scale=0.5, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=inside,
tick pos=left,
xmin=1000, xmax=5000,
xtick style={color=black},
xlabel={Number of Seeds ($C$)},
ylabel={Num of Augmented Data},
% ymode=log,
% log basis y={10},
ymin=0, ymax=22000,
ytick={0,10000,20000},
ytick style={color=black}
%title = {Training Time}
]
\addplot [thick, color0]
table {%
1000 2974
2000 4446
5000 5281
};
\addlegendentry{2D Classification}

\addplot [thick, color1]
table {%
1000 2997
2000 5962
5000 9468
};
\addlegendentry{Robot Handover}

\addplot [thick, color2]
table {%
1000 6505
2000 11010
5000 21020
};
\addlegendentry{Human Assembly}



\end{groupplot}
\end{tikzpicture}


==> supplement_img/C_time.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.1,0,0.95}
\definecolor{color1}{rgb}{1,0,0}
\definecolor{color2}{rgb}{1,0.498,0.0549}
\pgfplotsset{compat=1.5}
\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
width = \linewidth,
height =4cm,
font = \small,%\footnotesize,
legend cell align={left},
legend style={nodes={scale=0.6, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=inside,
tick pos=left,
xmin=500, xmax=5500,
xtick style={color=black},
xlabel={Number of Seeds ($C$)},
xtick={1000,2000,3000,4000,5000},
ylabel={Time (s)},
ymode=log,
log basis y={10},
ymin=0, ymax=10000,
ytick style={color=black}
%title = {Training Time}
]
\addplot [mark=triangle*, color0]
table {%
1000 66.505
2000 74.355
5000 86.424
};
\addlegendentry{2D Classification}

\addplot [mark=*, color1]
table {%
1000 1168.794
2000 1959
5000 6951
};
\addlegendentry{Robot Handover}

\addplot [mark=square*, color2]
table {%
1000 336.497
2000 533.373
5000 1022.944
};
\addlegendentry{Human Assembly}






\end{groupplot}
\end{tikzpicture}


==> supplement_img/rv_time.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.1,0,0.95}
\definecolor{color1}{rgb}{1,0,0}
\definecolor{color2}{rgb}{1,0.498,0.0549}
\pgfplotsset{compat=1.5}
\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
width = \linewidth,
height = 4cm,
font = \small,%\footnotesize,
legend cell align={left},
legend style={nodes={scale=0.6, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=inside,
tick pos=left,
xmin=0, xmax=1100,
xtick style={color=black},
xlabel={Inner Optimization Frequency ($r$)},
ylabel={Time (s)},
ymode=log,
log basis y={10},
ymin=0, ymax=20000,
ytick style={color=black}
%title = {Training Time}
]
\addplot[mark=triangle*,color0]
table {%
50 468.149
500 43.906
1000 39.141
};
\addlegendentry{2D Classification}

\addplot [mark=*, color1]
table {%
50 12895
500 395
1000 131.817
};
\addlegendentry{Robot Handover}

\addplot [mark=square*, color2]
table {%
50 5835.460
500 183.601
1000 94.250
};
\addlegendentry{Human Assembly}


\end{groupplot}
\end{tikzpicture}

